FairFly: A Fair Motion Planner for Fleets of Autonomous UAVs in Urban Airspace

We present a solution to the problem of fairly planning a fleet of Unmanned Aerial Vehicles (UAVs) that have different missions and operators, such that no one operator unfairly gets to finish its missions early at the expense of others - unless this was explicitly negotiated. When hundreds of UAVs share an urban airspace, the relevant authorities should allocate corridors to them such that they complete their missions, but no one vehicle is accidentally given an exceptionally fast path at the expense of another, which is thus forced to wait and waste energy. Our solution, FairFly, addresses the fair planning question for general autonomous systems, including UAV fleets, subject to complex missions typical of urban applications. FairFly formalizes each mission in temporal logic. An offline search finds the fairest paths that satisfy the missions and can be flown by the UAVs, leading to lighter online control load. It allows explicit negotiation between UAVs to enable imbalanced path durations if desired. We present three fairness notions, including one that reduces energy consumption. We validate our results in simulation, and demonstrate a lighter computational load and less UAV energy consumption as a result of flying fair trajectories.

==> STLrobustness <==

Formally, let $M=\{\mu_1,\ldots,\mu_L\}$ be a set of real-valued functions of the state $\mu_k:X \rightarrow \Re$.
%These functions are called \textit{booleanizers}.
For each $\mu_k$ define the \textit{atomic proposition} $p_k \defeq \mu_k(x) \geq 0$.
Set $AP \defeq \{p_1,\ldots,p_L\}$.
Each atomic proposition defines a set, namely, $p_k$ defines $\{x\in X\such \mu_k(x)\geq 0\}$.
Let $I  \subset \Re$ denote a non-singleton interval, $\top$ the Boolean True, $p$ a proposition, $\neg$ and $\land$ the Boolean negation and AND operators, respectively, and $\until$ the Until temporal operator.
An STL formula $\formula$ is built recursively from the propositions using the following grammar:
\[\formula \defeq \top|p|\neg \formula | \formula_1 \land \formula_2 | \formula_1 \until_I \formula_2\]

Following the Fly-by-Logic approach~\cite{pant2018fly}, we design a \textit{discrete-time }
Informally, $\formula_1 \until_I \formula_2$ means that $\formula_2$ must hold at some point in $I$, and \textit{until} then, $\formula_1$ must hold without interruption.
The disjunction ($\lor$), implication ($\implies$), Always ($\always$) and Eventually ($\eventually$) operators can be defined using the above operators.
Formally, the \textit{pointwise semantics} of an STL formula $\formula$ define what it means for a system trajectory $\sstraj$ to satisfy $\formula$.
%Let $\Oc: AP \rightarrow \Pc(X)$ be an \textit{observation} map for the atomic propositions.
\begin{definition}[STL semantics]
	\label{def:boolean sat}
	Let $\TDom = [0:dt:T]$. The boolean truth value of $\formula$ w.r.t. the discrete-time trajectory $\sstraj:\TDom \rightarrow X$ at time $t \in \TDom$ is defined recursively.	
	\begin{eqnarray*}
		\label{eq:boolean sat}
		(\sstraj,t) \models \top &\Leftrightarrow& \top
		\\
		\forall p_k \in AP, (\sstraj, t) \; \models p &\Leftrightarrow& \mu_k(x_t) \geq 0
		\\
		(\sstraj,t) \models \neg \formula&\Leftrightarrow& \neg (\sstraj,t) \models \formula
		\\
		(\sstraj,t) \models  \formula_1 \land \formula_2&\Leftrightarrow& (\sstraj,t) \models \formula_1 \land (\sstraj,t) \models \formula_2
		\\
		(\sstraj,t) \models \formula_1 \until_I \formula_2 &\Leftrightarrow& \exists t' \in (t+I)\cap \TDom .  (\sstraj,t') \models \formula_2  
		\\
		&& \, \land \forall t'' \in (t,t')\cap\TDom, \;\; (\sstraj,t'') \models \formula_1 
	\end{eqnarray*}
\end{definition}

We say $\sstraj$ \textit{satisfies} $\formula$ if $(\sstraj,0) \models \formula$.

\textit{All formulas that appear in this paper have bounded temporal intervals: $ 0\leq \inf I < \sup I < +\infty$.}
To evaluate whether such a \textit{bounded} formula $\formula$ holds on a given trajectory, only a finite-length prefix of that trajectory is needed.
Its length can be upper-bounded by the \textit{horizon} of $\formula$, $hrz(\formula) \in \Ne$, calculable as shown in~\cite{Raman14_MPCSTL}. 
For example, the horizon of $\always_{[0,2]}(\eventually_{[2,4]}p)$ is 2+4=6: we need to observe a trajectory of, at most, length 6 to determine whether the formula holds. 

Designing a controller that satisfies the STL formula $\formula$\footnote{Strictly, a controller s.t. the closed-loop behavior satisfies the formula.} is not always enough.
In a dynamic environment, where the system must react to new unforeseen events, it is useful to have a margin of maneuverability.
That is, it is useful to control the system such that we \textit{maximize} our degree of satisfaction of the formula.
When unforeseen events occur, the system can react to them without violating the formula.
This degree of satisfaction can be formally defined and computed using the \textit{robust semantics} of temporal logic~\cite{Donze10STLRob,FainekosP09tcs}.
\begin{definition}[Robustness\cite{FainekosP09tcs,Donze10STLRob}]
	\label{def:robustness estimate}
	The \emph{robustness} of STL formula $\varphi$ relative to $\sstraj:\TDom \rightarrow X$ at time $t \in \TDom$ is 
	\begin{eqnarray*}
		\label{eq:robustness estimate}
		\rob_{\top} (\sstraj,t) &=& +\infty
		\\
		\rob_{p_k} (\sstraj,t) &=& \mu_k(x_t)\,\forall p_k \in AP, \;  
		\\
		\rob_{\lnot \formula} (\sstraj,t) &=& - \rob_{\formula} (\sstraj,t)
		\\
		\rob_{ \formula_1 \land \formula_2} (\sstraj,t) &=& \rob_{\formula_1} (\sstraj,t) \sqcap \rob_{\formula_2} (\sstraj,t) 
		\\
		\rob_{ \formula_1 \until_I \formula_2} (\sstraj,t) &=& \sqcup_{t' \in (t+I)\cap \TDom} \left(\rob_{\formula_2} (\sstraj,t') \bigsqcap \right.
		\\
		&& \left. \sqcap_{t'' \in [t,t')\cap \TDom}   \rob_{\formula_1} (\sstraj,t'') \right) 
	\end{eqnarray*}
	When $t=0$, we write $\robf(\sstraj)$ instead of $\robf(\sstraj,0)$.
\end{definition}
The robustness is a real-valued function of $\sstraj$ with the following important property.
\begin{theorem} \cite{FainekosP09tcs}
	\label{thm:rob objective}
	For any $\sstraj \in \SigSpace$ and STL formula $\formula$, 
	if $\robf(\sstraj,t) <0$ then $\sstraj$ violates $\formula$ at time $t$, and if $\robf(\sstraj,t) > 0$ then $\sstraj$ satisfies $\formula$ at $t$. 
	The case $\robf(\sstraj,t) =0$ is inconclusive.
\end{theorem} 

Thus, we can compute control inputs by \textit{maximizing} the robustness over the set of finite input sequences of a certain length.
The obtained sequence $\inpSig^*$ is valid if $\robf(\sstraj^*,t)$ is positive, where $\sstraj^*$ and $\inpSig^*$ obey \eqref{eq:xt}.
The larger $\robf(\sstraj^*,t)$, the more robust is the behavior of the system: intuitively, $\sstraj^*$ can be disturbed and $\robf$ might decrease but not go negative.
In fact, the amount of disturbance that $\sstraj^*$ can sustain is precisely $\robf$: that is, if $\sstraj^* \models \formula$, then $\sstraj^*+e \models \formula$ for all disturbances $e:\TDom \rightarrow X$ s.t. $\sup_{t\in \TDom}\|e(t)\| <\robf(\sstraj^*)$.

If $\TDom=[0,T]$ then the above naturally defines satisfaction of $\formula$ by a \textit{continuous-time} trajectory $\outtraj_c:[0,T]\rightarrow X$.


==> STLrobustness.tex <==

Formally, let $M=\{\mu_1,\ldots,\mu_L\}$ be a set of real-valued functions of the state $\mu_k:X \rightarrow \Re$.
%These functions are called \textit{booleanizers}.
For each $\mu_k$ define the \textit{atomic proposition} $p_k \defeq \mu_k(x) \geq 0$.
Set $AP \defeq \{p_1,\ldots,p_L\}$.
Each atomic proposition defines a set, namely, $p_k$ defines $\{x\in X\such \mu_k(x)\geq 0\}$.
Let $I  \subset \Re$ denote a non-singleton interval, $\top$ the Boolean True, $p$ a proposition, $\neg$ and $\land$ the Boolean negation and AND operators, respectively, and $\until$ the Until temporal operator.
An STL formula $\formula$ is built recursively from the propositions using the following grammar:
\[\formula \defeq \top|p|\neg \formula | \formula_1 \land \formula_2 | \formula_1 \until_I \formula_2\]

Following the Fly-by-Logic approach~\cite{pant2018fly}, we design a \textit{discrete-time }
Informally, $\formula_1 \until_I \formula_2$ means that $\formula_2$ must hold at some point in $I$, and \textit{until} then, $\formula_1$ must hold without interruption.
The disjunction ($\lor$), implication ($\implies$), Always ($\always$) and Eventually ($\eventually$) operators can be defined using the above operators.
Formally, the \textit{pointwise semantics} of an STL formula $\formula$ define what it means for a system trajectory $\sstraj$ to satisfy $\formula$.
%Let $\Oc: AP \rightarrow \Pc(X)$ be an \textit{observation} map for the atomic propositions.
\begin{definition}[STL semantics]
	\label{def:boolean sat}
	Let $\TDom = [0:dt:T]$. The boolean truth value of $\formula$ w.r.t. the discrete-time trajectory $\sstraj:\TDom \rightarrow X$ at time $t \in \TDom$ is defined recursively.	
	\begin{eqnarray*}
		\label{eq:boolean sat}
		(\sstraj,t) \models \top &\Leftrightarrow& \top
		\\
		\forall p_k \in AP, (\sstraj, t) \; \models p &\Leftrightarrow& \mu_k(x_t) \geq 0
		\\
		(\sstraj,t) \models \neg \formula&\Leftrightarrow& \neg (\sstraj,t) \models \formula
		\\
		(\sstraj,t) \models  \formula_1 \land \formula_2&\Leftrightarrow& (\sstraj,t) \models \formula_1 \land (\sstraj,t) \models \formula_2
		\\
		(\sstraj,t) \models \formula_1 \until_I \formula_2 &\Leftrightarrow& \exists t' \in (t+I)\cap \TDom .  (\sstraj,t') \models \formula_2  
		\\
		&& \, \land \forall t'' \in (t,t')\cap\TDom, \;\; (\sstraj,t'') \models \formula_1 
	\end{eqnarray*}
\end{definition}

We say $\sstraj$ \textit{satisfies} $\formula$ if $(\sstraj,0) \models \formula$.

\textit{All formulas that appear in this paper have bounded temporal intervals: $ 0\leq \inf I < \sup I < +\infty$.}
To evaluate whether such a \textit{bounded} formula $\formula$ holds on a given trajectory, only a finite-length prefix of that trajectory is needed.
Its length can be upper-bounded by the \textit{horizon} of $\formula$, $hrz(\formula) \in \Ne$, calculable as shown in~\cite{Raman14_MPCSTL}. 
For example, the horizon of $\always_{[0,2]}(\eventually_{[2,4]}p)$ is 2+4=6: we need to observe a trajectory of, at most, length 6 to determine whether the formula holds. 

Designing a controller that satisfies the STL formula $\formula$\footnote{Strictly, a controller s.t. the closed-loop behavior satisfies the formula.} is not always enough.
In a dynamic environment, where the system must react to new unforeseen events, it is useful to have a margin of maneuverability.
That is, it is useful to control the system such that we \textit{maximize} our degree of satisfaction of the formula.
When unforeseen events occur, the system can react to them without violating the formula.
This degree of satisfaction can be formally defined and computed using the \textit{robust semantics} of temporal logic~\cite{Donze10STLRob,FainekosP09tcs}.
\begin{definition}[Robustness\cite{FainekosP09tcs,Donze10STLRob}]
	\label{def:robustness estimate}
	The \emph{robustness} of STL formula $\varphi$ relative to $\sstraj:\TDom \rightarrow X$ at time $t \in \TDom$ is 
	\begin{eqnarray*}
		\label{eq:robustness estimate}
		\rob_{\top} (\sstraj,t) &=& +\infty
		\\
		\rob_{p_k} (\sstraj,t) &=& \mu_k(x_t)\,\forall p_k \in AP, \;  
		\\
		\rob_{\lnot \formula} (\sstraj,t) &=& - \rob_{\formula} (\sstraj,t)
		\\
		\rob_{ \formula_1 \land \formula_2} (\sstraj,t) &=& \rob_{\formula_1} (\sstraj,t) \sqcap \rob_{\formula_2} (\sstraj,t) 
		\\
		\rob_{ \formula_1 \until_I \formula_2} (\sstraj,t) &=& \sqcup_{t' \in (t+I)\cap \TDom} \left(\rob_{\formula_2} (\sstraj,t') \bigsqcap \right.
		\\
		&& \left. \sqcap_{t'' \in [t,t')\cap \TDom}   \rob_{\formula_1} (\sstraj,t'') \right) 
	\end{eqnarray*}
	When $t=0$, we write $\robf(\sstraj)$ instead of $\robf(\sstraj,0)$.
\end{definition}
The robustness is a real-valued function of $\sstraj$ with the following important property.
\begin{theorem} \cite{FainekosP09tcs}
	\label{thm:rob objective}
	For any $\sstraj \in \SigSpace$ and STL formula $\formula$, 
	if $\robf(\sstraj,t) <0$ then $\sstraj$ violates $\formula$ at time $t$, and if $\robf(\sstraj,t) > 0$ then $\sstraj$ satisfies $\formula$ at $t$. 
	The case $\robf(\sstraj,t) =0$ is inconclusive.
\end{theorem} 

Thus, we can compute control inputs by \textit{maximizing} the robustness over the set of finite input sequences of a certain length.
The obtained sequence $\inpSig^*$ is valid if $\robf(\sstraj^*,t)$ is positive, where $\sstraj^*$ and $\inpSig^*$ obey \eqref{eq:xt}.
The larger $\robf(\sstraj^*,t)$, the more robust is the behavior of the system: intuitively, $\sstraj^*$ can be disturbed and $\robf$ might decrease but not go negative.
In fact, the amount of disturbance that $\sstraj^*$ can sustain is precisely $\robf$: that is, if $\sstraj^* \models \formula$, then $\sstraj^*+e \models \formula$ for all disturbances $e:\TDom \rightarrow X$ s.t. $\sup_{t\in \TDom}\|e(t)\| <\robf(\sstraj^*)$.

If $\TDom=[0,T]$ then the above naturally defines satisfaction of $\formula$ by a \textit{continuous-time} trajectory $\outtraj_c:[0,T]\rightarrow X$.

